Line Drawings from 3D Models

This tutorial describes the geometry and algorithms for generating line drawings from 3D models, focusing on occluding contours. The geometry of occluding contours on meshes and on smooth surfaces is described in detail, together with algorithms for extracting contours, computing their visibility, and creating stylized renderings and animations. Exact methods and hardware-accelerated fast methods are both described, and the trade-offs between different methods are discussed. The tutorial brings together and organizes material that, at present, is scattered throughout the literature. It also includes some novel explanations, and implementation tips. A thorough survey of the field of non-photorealistic 3D rendering is also included, covering other kinds of line drawings and artistic shading.

==> figures/smooth_contours/volume_thickness.pdf_tex.tex <==
%% Creator: Inkscape inkscape 0.92.2, www.inkscape.org
%% PDF/EPS/PS + LaTeX output extension by Johan Engelen, 2010
%% Accompanies image file 'volume_thickness.pdf' (pdf, eps, ps)
%%
%% To include the image in your LaTeX document, write
%%   \input{<filename>.pdf_tex}
%%  instead of
%%   \includegraphics{<filename>.pdf}
%% To scale the image, write
%%   \def\svgwidth{<desired width>}
%%   \input{<filename>.pdf_tex}
%%  instead of
%%   \includegraphics[width=<desired width>]{<filename>.pdf}
%%
%% Images with a different path to the parent latex file can
%% be accessed with the `import' package (which may need to be
%% installed) using
%%   \usepackage{import}
%% in the preamble, and then including the image with
%%   \import{<path to file>}{<filename>.pdf_tex}
%% Alternatively, one can specify
%%   \graphicspath{{<path to file>/}}
%% 
%% For more information, please see info/svg-inkscape on CTAN:
%%   http://tug.ctan.org/tex-archive/info/svg-inkscape
%%
\begingroup%
  \makeatletter%
  \providecommand\color[2][]{%
    \errmessage{(Inkscape) Color is used for the text in Inkscape, but the package 'color.sty' is not loaded}%
    \renewcommand\color[2][]{}%
  }%
  \providecommand\transparent[1]{%
    \errmessage{(Inkscape) Transparency is used (non-zero) for the text in Inkscape, but the package 'transparent.sty' is not loaded}%
    \renewcommand\transparent[1]{}%
  }%
  \providecommand\rotatebox[2]{#2}%
  \ifx\svgwidth\undefined%
    \setlength{\unitlength}{147.4015748bp}%
    \ifx\svgscale\undefined%
      \relax%
    \else%
      \setlength{\unitlength}{\unitlength * \real{\svgscale}}%
    \fi%
  \else%
    \setlength{\unitlength}{\svgwidth}%
  \fi%
  \global\let\svgwidth\undefined%
  \global\let\svgscale\undefined%
  \makeatother%
  \begin{picture}(1,0.59615385)%
    \put(0,0){\includegraphics[width=\unitlength,page=1]{volume_thickness.pdf}}%
    \put(0.50517906,0.5431374){\color[rgb]{0,0,0}\makebox(0,0)[b]{\smash{$R-T$}}}%
    \put(0.44186124,0.23142764){\color[rgb]{0,0,0}\makebox(0,0)[lb]{\smash{$R$}}}%
    \put(0.20648708,0.44988038){\color[rgb]{0,0,0}\makebox(0,0)[lb]{\smash{$\theta_T$}}}%
    \put(0.69199506,0.34668696){\color[rgb]{0,0,0}\rotatebox{-90}{\makebox(0,0)[b]{\smash{$\sqrt{2RT-T^2}$}}}}%
    \put(0.80483352,0.00498546){\color[rgb]{0,0,0}\makebox(0,0)[b]{\smash{$T$}}}%
    \put(0.96063485,0.17880126){\color[rgb]{0,0,0}\makebox(0,0)[b]{\smash{$\vec{v}$}}}%
    \put(0.94982195,0.51460728){\color[rgb]{0,0,0}\makebox(0,0)[lb]{\smash{$\vec{n}$}}}%
    \put(0.93437653,0.04282696){\color[rgb]{0,0,0}\makebox(0,0)[lb]{\smash{$\vec{n}_\text{max}$}}}%
    \put(0,0){\includegraphics[width=\unitlength,page=2]{volume_thickness.pdf}}%
  \end{picture}%
\endgroup%


==> figures/smooth_contours/volume_transferfunc.pdf_tex.tex <==
%% Creator: Inkscape inkscape 0.92.2, www.inkscape.org
%% PDF/EPS/PS + LaTeX output extension by Johan Engelen, 2010
%% Accompanies image file 'implicit_transferfunc.pdf' (pdf, eps, ps)
%%
%% To include the image in your LaTeX document, write
%%   \input{<filename>.pdf_tex}
%%  instead of
%%   \includegraphics{<filename>.pdf}
%% To scale the image, write
%%   \def\svgwidth{<desired width>}
%%   \input{<filename>.pdf_tex}
%%  instead of
%%   \includegraphics[width=<desired width>]{<filename>.pdf}
%%
%% Images with a different path to the parent latex file can
%% be accessed with the `import' package (which may need to be
%% installed) using
%%   \usepackage{import}
%% in the preamble, and then including the image with
%%   \import{<path to file>}{<filename>.pdf_tex}
%% Alternatively, one can specify
%%   \graphicspath{{<path to file>/}}
%% 
%% For more information, please see info/svg-inkscape on CTAN:
%%   http://tug.ctan.org/tex-archive/info/svg-inkscape
%%
\begingroup%
  \makeatletter%
  \providecommand\color[2][]{%
    \errmessage{(Inkscape) Color is used for the text in Inkscape, but the package 'color.sty' is not loaded}%
    \renewcommand\color[2][]{}%
  }%
  \providecommand\transparent[1]{%
    \errmessage{(Inkscape) Transparency is used (non-zero) for the text in Inkscape, but the package 'transparent.sty' is not loaded}%
    \renewcommand\transparent[1]{}%
  }%
  \providecommand\rotatebox[2]{#2}%
  \ifx\svgwidth\undefined%
    \setlength{\unitlength}{96.37795276bp}%
    \ifx\svgscale\undefined%
      \relax%
    \else%
      \setlength{\unitlength}{\unitlength * \real{\svgscale}}%
    \fi%
  \else%
    \setlength{\unitlength}{\svgwidth}%
  \fi%
  \global\let\svgwidth\undefined%
  \global\let\svgscale\undefined%
  \makeatother%
  \begin{picture}(1,0.88235294)%
    \put(0,0){\includegraphics[width=\unitlength,page=1]{volume_transferfunc.pdf}}%
    \put(0.1120998,0.83112881){\color[rgb]{0,0,0}\makebox(0,0)[lb]{\smash{$\vec{v} \cdot \vec{n}$}}}%
    \put(0.94322854,0.39304337){\color[rgb]{0.17254902,0.17254902,0.17254902}\makebox(0,0)[lb]{\smash{$\kappa_r$}}}%
    \put(0.04924459,0.77822592){\color[rgb]{0,0,0}\makebox(0,0)[rb]{\smash{1}}}%
    \put(0.04790204,0.39697385){\color[rgb]{0,0,0}\makebox(0,0)[rb]{\smash{0}}}%
    \put(0.04924459,-0.00000004){\color[rgb]{0,0,0}\makebox(0,0)[rb]{\smash{-1}}}%
    \put(0,0){\includegraphics[width=\unitlength,page=2]{volume_transferfunc.pdf}}%
  \end{picture}%
\endgroup%


==> frontmatter.tex <==
%% Front matter for for FnT Computer Graphics & Vision
%% (c) 2013 Neal Parikh (Stanford University)
%% 
%% Based on earlier NOW style files by S. Kumar,
%% J. Sebastian, T. Hoekwater, and B.V. Elvenkind

\RequirePackage{lastpage}
\RequirePackage{multicol}

% base journal information definitions
\def\doi#1{\def\@doi{#1}}
\def\copyrightowner#1{\def\@copyrightowner{#1}}
\def\firstpage#1{\def\@firstpage{#1}}
\def\isbn#1{\def\@isbn{#1}}
\def\issue#1{\def\@issue{#1}}
\def\journalinfofont{\fontsize{8}{10}\selectfont\rmfamily}
\def\journallibraryinfo#1{\def\@libraryinfo{#1}}
\def\journaltitle#1{\def\@journaltitle{#1}}
\def\journaltitleprefix#1{\def\@journaltitleprefix{#1}}
\def\@lastpage{\pageref{LastPage}}
\def\lastpage#1{\def\@lastpage{#1}}
\def\copyrightyear#1{\def\@copyrightyear{#1}}
\edef\@copyrightyear{\the\year}
\def\pubyear#1{\def\@pubyear{#1}}
\edef\@pubyear{\the\year}
\def\volume#1{\def\@volume{#1}}

\def\journaltopicintro#1{\def\@journaltopicintro{#1}}
\def\journaltopics#1{\def\@journaltopics{#1}}

% editors
\newcount\editorcount
\def\@editors{}
\def\journaleditor#1{%
  \advance\editorcount1 
  \ifx\empty\@editors
    \def\@editors{#1}%
  \else
    \expandafter\def\expandafter\@editors\expandafter{\@editors\\[0.3em]#1}%
  \fi
}

% editors in chief
\newcount\chiefeditorcount
\def\@chiefeditors{}
\def\journalchiefeditor#1{%
  \advance\chiefeditorcount1 
  \ifx\empty\@chiefeditors
    \def\@chiefeditors{#1}%
  \else
    \expandafter\def\expandafter\@chiefeditors\expandafter{\@chiefeditors\\[1em]#1}%
  \fi
}

%% title page

\renewcommand\maketitle{\begin{titlepage}%

\if@openright % -- for 'book' version
\parindent \z@

% title page
\thispagestyle{empty}
\vspace*{\fill}
\begin{flushright}
\begin{minipage}{0.8\textwidth}
\begin{flushright}
\renewcommand{\baselinestretch}{1.1}
\sffamily\bfseries\huge 
\@title
\end{flushright}
\end{minipage}
\end{flushright}
\vspace*{\fill}

% title+author page
\cleardoublepage
\thispagestyle{empty}

\begin{flushright}
{\renewcommand{\baselinestretch}{1.2}
\sffamily\Huge\bfseries \@title\par}
\vspace{3ex}
\noindent\rule{\textwidth}{2pt}
\vspace{1ex}\par

\begingroup
\def\and{%
  \end{tabular}%
  \par\vspace*{1.5ex}
  \begin{tabular}[t]{r@{}}
  \bfseries}

  \fontsize{13}{15}\selectfont\sffamily
\begin{tabular}[t]{r@{}}
    \bfseries
    \@author
\end{tabular}
\endgroup
\vfill
\includegraphics[width=53bp]{now_logo}\\
\includegraphics[width=81bp]{essence_logo}\\
Boston --- Delft
\end{flushright}

% publisher page
\newpage
\thispagestyle{empty}
\begingroup

\begin{minipage}{\textwidth}
\bfseries\sffamily\Large \@journaltitleprefix\\ \@journaltitle
\end{minipage}

\parskip6pt


\vfill

{\itshape Published, sold and distributed by:}\\
now Publishers Inc.\\
PO Box 1024\\
Hanover, MA\ 02339\\
United States\\
Tel.\ +1-781-985-4510\\
www.nowpublishers.com\\
sales@nowpublishers.com

{\itshape Outside North America:}\\
now Publishers Inc.\\
PO Box 179\\
2600 AD Delft\\
The Netherlands\\
Tel.\ +31-6-51115274

The preferred citation for this publication is

{\raggedright
\@copyrightowner. \emph{\@title}.  \@journaltitleprefix\
\@journaltitle, vol.~\@volume, no.~\@issue, pp.~\@firstpage--\@lastpage,
\@pubyear.\par}

{\itshape This Foundations and Trends\textsuperscript{\textregistered} issue
was typeset in \LaTeX\ using a class file designed by Neal Parikh. Printed on
acid-free paper.}

ISBN: \@isbn\\ \copyright\ \@copyrightyear\ \@copyrightowner

\vfill

\fontsize{8}{9}\selectfont
All rights reserved. No part of this publication may be
reproduced, stored in a retrieval system, or transmitted in any form
or by any means, mechanical, photocopying, recording or otherwise,
without prior written permission of the publishers.

Photocopying. In the USA: This journal is registered at the Copyright
Clearance Center, Inc., 222 Rosewood Drive, Danvers, MA 01923. 
Authorization to photocopy items for
internal or personal use, or the internal or personal use of specific
clients, is granted by now Publishers Inc for users registered with 
the Copyright Clearance Center (CCC).
The `services' for users can be found on the internet at:
www.copyright.com

For those organizations that have been granted a photocopy license, a
separate system of payment has been arranged. Authorization does not
extend to other kinds of copying, such as that for general
distribution, for advertising or promotional purposes, for creating
new collective works, or for resale.  In the rest of the world:
Permission to photocopy must be obtained from the copyright
owner. Please apply to now Publishers Inc., PO Box 1024, Hanover, MA
02339, USA; Tel. +1 781 871 0245; www.nowpublishers.com;
sales@nowpublishers.com

now Publishers Inc. has an exclusive license to publish this
material worldwide. Permission to use this content must be obtained from
the copyright license holder. Please apply to now Publishers, PO Box 179, 2600
AD Delft, The Netherlands, www.nowpublishers.com; e-mail:
sales@nowpublishers.com\par
\endgroup

% editorial board
\newpage
\thispagestyle{empty}
\begin{center}
\sffamily\LARGE
{\bfseries \@journaltitleprefix\\ \@journaltitle}\\
{Volume \@volume, Issue \@issue, \@pubyear}\\
{\bfseries Editorial Board}
\end{center}

\vspace{8pt}

\ifnum\chiefeditorcount>1
{\sffamily\bfseries Editors-in-Chief}
{
\begin{multicols}{2}
\@chiefeditors
\end{multicols}}
\else
{\sffamily\bfseries Editor-in-Chief}\par
\vspace*{10pt}
\begin{footnotesize}
\begin{tabular}[t]{@{}l}
\@chiefeditors \\
\end{tabular}
\end{footnotesize}
\vspace*{10pt}
\fi

{\sffamily \bfseries Editors}
{\fontsize{9}{11}\selectfont
\begin{multicols}{3}
\raggedcolumns
\@editors
\end{multicols}}%

% editorial scope
\newpage % page vi -- blank
\thispagestyle{empty}
\begin{center}
{\sffamily\bfseries\LARGE Editorial Scope}
\end{center}

\vspace{18pt}

{\bfseries\large\sffamily Topics}\\

\@journaltopicintro\par

\fontsize{10}{13}\selectfont
\begin{multicols}{2}
    \raggedright
    \@journaltopics
\end{multicols}

{\bfseries\large\sffamily Information for Librarians}\\

\@libraryinfo\par

\else\fi % -- no book front matter for "journal" version

% -- end book front matter

% title+author page
\newpage
\thispagestyle{empty}
\hbox to \textwidth{%
    \vbox{\raggedright
    \hsize=.6\textwidth \journalinfofont
{\hangindent=3.5ex
\hangafter=1
\@journaltitleprefix\\ \@journaltitle\par}%
Vol.~\@volume, No.~\@issue\ (\@pubyear) 
\@firstpage--\@lastpage\\
{\hangindent=3.5ex
\hangafter=1
\copyright\ \@copyrightyear\ \@copyrightowner\par}%
DOI: \@doi}\hss
\vbox{\hsize=.4\textwidth 
    \raggedleft
    \includegraphics[width=53bp]{now_logo}\\
    \includegraphics[width=81bp]{essence_logo}\\
    \par
}}\par
\let\footnoterule\relax
\let\footnote\thanks
\null\vfil
\vskip 60\p@
\begin{center}%
{\LARGE \sffamily \bfseries \@title \par}%
\vskip 3em%
{
\large
\lineskip .75em%
     \lineskip .75em%
      \begin{tabular}[t]{c}%
        \@author
      \end{tabular}\par}%
\end{center}\par
\@thanks
\vfill
\end{titlepage}
\setcounter{footnote}{0}%
}

%% defaults and settings for this FnT

\def\@copyrightowner{now Publishers Inc.}
\journaltitleprefix{Foundations and Trends\textsuperscript{\textregistered} in}
\volume{XX}
\issue{XX}
\firstpage{1}
\isbn{XXX-X-XXXXX-XXX-X}
\doi{10.1561/XXXXXXXXXX}

\journaltitle{Computer Graphics and Vision}

\journalchiefeditor{\textbf{Brian Curless} \\
University of Washington}

\journalchiefeditor{\textbf{William T. Freeman}\\
Massachusetts Institute of Technology\columnbreak}

\journalchiefeditor{\textbf{Luc Van Gool} \\
KU Leuven and ETH Zurich}


\journaleditor{Marc Alexa \\ \emph{TU Berlin}}
\journaleditor{Kavita Bala \\ \emph{Cornell University}}
\journaleditor{Ronen Basri \\ \emph{Weizmann Institute}}
\journaleditor{Peter Belhumeur \\ \emph{Columbia University}}
\journaleditor{Andrew Blake \\ \emph{Microsoft Research}}
\journaleditor{Chris Bregler \\ \emph{Facebook/Oculus}}
\journaleditor{Joachim Buhmann \\ \emph{ETH Zurich}}
\journaleditor{Michael Cohen \\ \emph{Microsoft Research}}
\journaleditor{Paul Debevec \\ \emph{USC ICT}}
\journaleditor{Julie Dorsey \\ \emph{Yale University}}
\journaleditor{Fredo Durand \\ \emph{MIT}}
\journaleditor{Olivier Faugeras \\ \emph{INRIA}}
\journaleditor{Rob Fergus \\ \emph{New York University}}
\journaleditor{Mike Gleicher \\ \emph{University of Wisconsin}}
\journaleditor{Richard Hartley \\ \emph{ANU}}
\journaleditor{Aaron Hertzmann \\ \emph{Adobe Research, USA}}
\journaleditor{Hugues Hoppe \\ \emph{Microsoft Research}}
\journaleditor{C. Karen Liu \\ \emph{Georgia Tech}}
\journaleditor{David Lowe \\ \emph{UBC}}
\journaleditor{Jitendra Malik \\ \emph{UC Berkeley}}
\journaleditor{Steve Marschner \\ \emph{Cornell University}}
\journaleditor{Shree Nayar \\ \emph{Columbia University}}
\journaleditor{James O'Brien \\ \emph{UC Berkeley}}
\journaleditor{Tomas Pajdla \\ \emph{Czech TU}}
\journaleditor{Pietro Perona \\ \emph{Caltech}}
\journaleditor{Marc Pollefeys \\ \emph{ETH Zurich}}
\journaleditor{Jean Ponce \\ \emph{Ecole Normale Sup\'erieure}}
\journaleditor{Long Quan \\ \emph{HKUST}}
\journaleditor{Cordelia Schmid \\ \emph{INRIA}}
\journaleditor{Steve Seitz \\ \emph{University of Washington}}
\journaleditor{Amnon Shashua \\ \emph{Hebrew University}}
\journaleditor{Peter Shirley \\ \emph{University of Utah}}
\journaleditor{Noah Snavely \\ \emph{Cornell University}}
\journaleditor{Stefano Soatto \\ \emph{UCLA}}
\journaleditor{Richard Szeliski \\ \emph{Microsoft Research}}
\journaleditor{Joachim Weickert \\ \emph{Saarland University}}
\journaleditor{Song Chun Zhu \\ \emph{UCLA}}
\journaleditor{Andrew Zisserman \\ \emph{University of Oxford}}

\journaltopicintro{\@journaltitleprefix\ \@journaltitle\ publishes
survey and tutorial articles in the following topics:}

\journaltopics{
\begin{itemize}\itemsep=0pt
    \item{Rendering}
    \item{Shape}
    \item{Mesh simplification}
    \item{Animation}
    \item{Sensors and sensing}
    \item{Image restoration and enhancement}
    \item{Segmentation and grouping}
    \item{Feature detection and selection}
    \item{Color processing}
    \item{Texture analysis and synthesis}
    \item{Illumination and reflectance modeling}
    \item{Shape representation}
    \item{Tracking}
    \item{Calibration}
    \item{Structure from motion}
    \item{Motion estimation and registration}
    \item{Stereo matching and reconstruction}
    \item{3D reconstruction and image-based modeling}
    \item{Learning and statistical methods}
    \item{Appearance-based matching}
    \item{Object and scene recognition}
    \item{Face detection and recognition}
    \item{Activity and gesture recognition}
    \item{Image and video retrieval}
    \item{Video analysis and event recognition}
    \item{Medical image analysis}
    \item{Robot localization and navigation}
\end{itemize}
}

\journallibraryinfo{%
  Foundations and Trends\textsuperscript{\textregistered} in \@journaltitle, \@pubyear,
  Volume~\@volume, 4 issues. ISSN paper version 1572-2740. %%% (\@paperprice).
  ISSN online version 1572-2759. %%% (\@onlineprice).
  Also available as a combined paper and online
  subscription.%%% (\@combinedprice).
}

\endinput

